Prospects for constrained supersymmetry at $\sqrt{s}=33$ TeV and $\sqrt{s}=100$ TeV proton-proton super-colliders

Discussions are underway for a high-energy proton-proton collider. Two preliminary ideas are the $\sqrt{s}=33$ TeV HE-LHC and the $\sqrt{s}=100$ TeV VLHC. With Bayesian statistics, we calculate the probabilities that the LHC, HE-LHC and VLHC discover SUSY in the future, assuming that nature is described by the CMSSM and given the experimental data from the LHC, LUX and Planck. We find that the LHC with $300$/fb at $\sqrt{s}=14$ TeV has a $15$-$75%$ probability of discovering SUSY. Should that run fail to discover SUSY, the probability of discovering SUSY with $3000$/fb is merely $1$-$10%$. Were SUSY to remain undetected at the LHC, the HE-LHC would have a $35$-$85%$ probability of discovering SUSY with $3000$/fb. The VLHC, on the other hand, ought to be definitive; the probability of it discovering SUSY, assuming that the CMSSM is the correct model, is $100%$.

==> preamble.tex <==
% Hyperlinks in document.
\usepackage{hyperref}

% Figures & tables.
\usepackage{graphicx}
 
% Italic captions for figures and tables with bold numbers.
\usepackage[font=small,labelfont=bf]{caption}
\captionsetup[figure]{textfont=it} 
\captionsetup[table]{textfont=it}
\usepackage{subfig}

% Hyphenation rules.
\usepackage[english]{babel}

% To avoid trailing \ on macros.
\usepackage{xspace}

% In-line lists.
\usepackage{paralist}

% Fonts.
\usepackage{microtype}
\usepackage{fouriernc}
\usepackage[scale=0.92]{tgschola}
\usepackage[T1]{fontenc}
\usepackage{bm} % Bold math.

% Custom enumerate environment.
\usepackage{enumitem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% New and renewcommand with math and xspace.
\newcommand{\mxnewcommand}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}
\newcommand{\mxrenewcommand}[2]{\renewcommand{#1}{\ensuremath{#2}\xspace}}

% New and renewcommand with  xspace.
\newcommand{\xnewcommand}[2]{\newcommand{#1}{#2\xspace}}
\newcommand{\xrenewcommand}[2]{\renewcommand{#1}{#2\xspace}}

% Units.
\mxnewcommand{\gev}{\,\text{GeV}}
\mxnewcommand{\tev}{\,\text{TeV}}
\mxnewcommand{\invfb}{/\text{fb}}

% LHC energies root(s) = X TeV.
\newcommand{\roots}[1]{\ensuremath{\sqrt{s}={#1}\tev}}

% Parameters.
\mxnewcommand{\msinglet}{m_S}
\mxnewcommand{\mhalf}{m_{1/2}}
\mxnewcommand{\mzero}{m_0}
\mxnewcommand{\azero}{A_0}
\mxnewcommand{\tanb}{\tan\beta}
\mxnewcommand{\sgnmu}{\text{sign}\,\mu}
\mxnewcommand{\mueff}{\mu_\text{eff}}
\mxnewcommand{\sgnmueff}{\text{sign}\,\mueff}
\mxnewcommand{\sgnb}{\text{sign}\,b}
\mxnewcommand{\msbar}{\overline{\text{MS}}}
\mxnewcommand{\invalpha}{1/\alpha_{\text{em}}(M_Z)^{\msbar}}
\mxnewcommand{\alphas}{\alpha_s(M_Z)^{\msbar}}
\mxnewcommand{\mt}{m_t^\text{Pole}}
\mxnewcommand{\mb}{m_b(m_b)^{\msbar} }
\mxnewcommand{\mz}{M_Z}
\mxnewcommand{\mhu}{m_{H_u}}
\mxnewcommand{\mhd}{m_{H_d}}
\mxnewcommand{\tanbsq}{\tan^2\beta}
\mxnewcommand{\mplanck}{M_\text{P}}
\mxnewcommand{\mgut}{M_\text{GUT}}
\mxnewcommand{\msusy}{M_\text{SUSY}}
\mxnewcommand{\mweak}{M_Z}

% CP symmetry.
\mxnewcommand{\cp}{\mathcal{CP}}

% Shorthand nuisance parameters.
\mxnewcommand{\mts}{m_t}
\mxnewcommand{\mbs}{m_b}
\mxnewcommand{\invalphas}{1/\alpha_{\text{em}} }
\mxnewcommand{\alphass}{\alpha_s}

% Lagrangian.
\newcommand{\lag}[1][]{\ensuremath{%
\mathcal{L}_\text{#1}%
}}
\newcommand{\superp}[1][]{\ensuremath{%
\mathcal{W}^\text{#1}%
}}
\mxnewcommand{\cc}{\text{c.c.}}


% Brackets - this is handy.
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}

% Statistical terms.
\mxnewcommand{\like}{\mathcal{L}}
\mxnewcommand{\prior}{\pi}
\mxnewcommand{\params}{m}
\mxnewcommand{\ev}{\mathcal{Z}}
\mxnewcommand{\point}{\vec{x}}
\mxnewcommand{\model}{\text{model}}
\mxnewcommand{\data}{\text{data}}
\mxnewcommand{\pd}{\,\prod\text{d}}

% Statistical functions
\newcommand{\priorf}[1]{\ensuremath{\prior(#1)}}
\newcommand{\likef}[1]{\ensuremath{\like(#1)}}
\newcommand{\gaussian}[3]{\ensuremath{\exp \[-\frac{\(#1 - #2\)^2}{2#3} \]}}
\newcommand{\pg}[2]{\ensuremath{p(#1\,\bm{|}\,#2)}}
\newcommand{\p}[1]{\ensuremath{p(#1)}}

% Partial derivative.
\newcommand{\dpartial}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\indpartial}[2]{\ensuremath{{\partial #1}/{\partial #2}}}

% Particle names.
\newcommand{\s}[1]{\ensuremath{\tilde{#1}}}
\newcommand{\sbar}[1]{\ensuremath{\tilde{\bar{#1}}}}
\newcommand{\sd}[1]{\ensuremath{\tilde{#1}^\dagger}}
\newcommand{\sbd}[1]{\ensuremath{\tilde{\bar{#1}}^\dagger}}
\newcommand{\neut}[1]{\ensuremath{{\chi}^0_{#1}}}
\newcommand{\charg}[1]{\ensuremath{{\chi}^\pm_{#1}}}

% Masses.
\newcommand{\ms}[1]{\ensuremath{m_{\s{#1}}}}
\newcommand{\mneut}[1]{\ensuremath{m_{\neut{#1}}}}
\newcommand{\mcharg}[1]{\ensuremath{m_{\charg{#1}}}}

% Constraints etc.
\mxnewcommand{\sigsip}{\sigma^{\text{SI}}_p}
\mxnewcommand{\abund}{\Omega h^2}
\newcommand{\br}[1]{\ensuremath{\text{BR}}(#1)}
\mxnewcommand{\bsg}{\br{B_s\to X_s\gamma}}
\mxnewcommand{\bsmm}{\br{B_s\to \mu\mu}}
\mxnewcommand{\btn}{\br{B_u\to \tau\nu}}
\mxnewcommand{\damu}{\delta a_\mu}
\mxnewcommand{\mh}{m_h}
\mxnewcommand{\ma}{m_A}
\mxnewcommand{\mw}{M_W}
\mxnewcommand{\dmbs}{\Delta M_{B_s}}
\mxnewcommand{\sineff}{\sin^{2} \theta_{\ell,\text{eff}}}

% Parameter planes.
\mxnewcommand{\pmm}{(\mzero,\,\mhalf)}
\mxnewcommand{\pat}{(\azero,\,\tanb)}
\mxnewcommand{\pcs}{(\mneut{1},\,\sigsip)}
\mxnewcommand{\pkm}{(\kappa,\,\msinglet)}
\mxnewcommand{\pmmu}{(\mzero,\,\mu)}
\xnewcommand{\stauc}{stau-coannihilation}
\xnewcommand{\Stauc}{Stau-coannihilation}

% Abbreviations.
\let\oldcite\cite
\renewcommand{\cite}{~\oldcite}
\newcommand{\reftable}[1]{Table~\ref{#1}} 
\newcommand{\reffig}[1]{Fig.~\ref{#1}}
\newcommand{\reffigs}[2]{Figs.~\ref{#1} and \ref{#2} } 
\newcommand{\refeq}[1]{Eq.~(\ref{#1})}
\newcommand{\refsec}[1]{Sec.~\ref{#1}}
\newcommand{\refcite}[1]{Ref.\cite{#1}}
\xnewcommand{\eg}{\textit{e.g.,}}
\xnewcommand{\ie}{\textit{i.e.,}}
\xnewcommand{\latincf}{\textit{c.f.,}}
\newcommand{\latin}[1]{\textit{#1}}
\mxnewcommand{\dash}{\text{, }}
\newcommand{\ic}[1]{``#1''}

% Shortcuts
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{ \end{equation}}
% Sientific notation.
\newcommand{\pn}[2]{\ensuremath{#1\cdot10^{#2}}} 
% See a paper.
\newcommand{\see}[1]{(see \eg\cite{#1})}
